Canadian Traveller Problems in Temporal Graphs

This paper formalises the Canadian Traveller problem as a positional two-player game on graphs. We consider two variants depending on whether an edge is blocked. In the locally-informed variant, the traveller learns if an edge is blocked upon reaching one of its endpoints, while in the uninformed variant, they discover this only when the edge is supposed to appear. We provide a polynomial algorithm for each shortest path variant in the uninformed case. This algorithm also solves the case of directed acyclic non-temporal graphs. In the locally-informed case, we prove that finding a winning strategy is PSPACE-complete. Moreover, we establish that the problem is polynomial-time solvable when $k=1$ but NP-hard for $k\geq 2$. Additionally, we show that the standard (non-temporal) Canadian Traveller Problem is NP-hard when there are $k\geq 4$ blocked edges, which is, to the best of our knowledge, the first hardness result for CTP for a constant number of blocked edges.

==> CONCLUSION/current.tex <==
\section{Conclusion}


We focus on the Canadian Traveller Problem in the temporal graph. This paper formalizes this problem as a positional game in two-player graphs: Traveler aims to reach a destination while BLocker intents on preventing them. We have proven that finding a winning strategy for Traveler is polynomial when the graph is acyclic (this result also holds for a non-temporal graph). However, for a cyclic topology, this problem becomes PSPACE-complete. One direction is to understand if we can construct parameterized algorithms. There are two types of approaches: either utilizing the topology of the static underlying graph (such as treewidth, the feedback vertex number)  or employing purely temporal parameters (such as interval-membership-width, constraints on \textcolor{blue}{régularité d'apparitions des arêtes}  ("the appearance regularity) of edges in the static underlying graph").
 
\textcolor{blue}{Peut-etre dire de faire la meme démarche pour le cas non-temporel à cause du Théorème 4} 
